Distributed Speculative Inference (DSI): Speculation Parallelism for Provably Faster Lossless Language Model Inference

This paper introduces distributed speculative inference (DSI), a novel inference algorithm that is provably faster than speculative inference (SI) [leviathan2023, chen2023, miao2024, sun2025, timor2025] and standard autoregressive inference (non-SI). Like other SI algorithms, DSI operates on frozen language models (LMs), requiring no training or architectural modifications, and it preserves the target distribution. Prior studies on SI have demonstrated empirical speedups over non-SI--but rely on sufficiently fast and accurate drafters, which are often unavailable in practice. We identify a gap where SI can be slower than non-SI if drafters are too slow or inaccurate. We close this gap by proving that DSI is faster than both SI and non-SI--given any drafters. DSI is therefore not only faster than SI, but also unlocks the acceleration of LMs for which SI fails. DSI leverages speculation parallelism (SP), a novel type of task parallelism, to orchestrate target and drafter instances that overlap in time, establishing a new foundational tradeoff between computational resources and latency. Our simulations show that DSI is 1.29-1.92x faster than SI in single-node setups for various off-the-shelf LMs and tasks. We open-source all our code.

==> illustration/benchmark.tex <==
\begin{tabular}{lrrrrr}
    \toprule
     & t0=0 & t1 & t2 & t3 & t4 \\
    \midrule
    non-SI & 0 & 2 & 4 & 8 & 9 \\
    SI worst case & 0 & 1 & 4 & 8 & 9 \\
    SI best case & 0 & 2 & 8 & 14 & 16 \\
    DSI worst case & 0 & 2 & 4 & 8 & 9 \\
    DSI best case & 0 & 8 & 26 & 50 & 58 \\
    \bottomrule
\end{tabular}
